Enumerating regular languages in radix order : Revisiting the Ackerman-Shallit algorithm

We consider the problem of enumerating a regular language $L$ in radix order, or more precisely, the equivalent problem of enumerating all words in $L$ of a given length in lexicographic order. Ackerman and Shallit gave in 2009 the principles of an efficient solution to this problem, but they did not use the enumeration complexity framework for their analysis. We adapt their work into an explicit algorithm that fits this framework.

==> aux/macros.tex <==
\newcommand{\arobase}{\raisebox{-0.2ex}{\fontfamily{ptm}\selectfont @}}
\newcommand{\mel}[2]{{\tt\href{mailto:#1@#2}{#1\arobase{}#2}}}

\makeatletter
\newcommand{\vm@date@separator}{\hspace*{0.15ex}\rule[0.4\vm@date@height]{1ex}{0.07\vm@date@height}\hspace*{0.15ex}}
\newcommand{\vmdatefont}[1]{#1}
\newcommand{\isotoday}{%
  \vmdatefont{
    \newdimen\vm@date@height%
    \setbox0=\hbox{0123456789}%
    \vm@date@height=\ht0 \advance\vm@date@height by -\dp0
    \the\year\vm@date@separator\two@digits{\month}\vm@date@separator\two@digits{\day}%
  }%
}

\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Dc}{\mathcal{D}}

\newcommand{\powerset}{\mathcal{P}}

\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}

\DeclareMathOperator{\incoming}{\mathop{\text{\normalfont\textsc{In}}}}
\DeclareMathOperator{\outgoing}{\mathop{\text{\normalfont\textsc{Out}}}}
\DeclareMathOperator{\indeg}{\mathop{\text{\normalfont\textsc{InDeg}}}}
\DeclareMathOperator{\outdeg}{\mathop{\text{\normalfont\textsc{OutDeg}}}}
\DeclareMathOperator{\src}{\mathop{\text{\normalfont\textsc{Src}}}}
\DeclareMathOperator{\tgt}{\mathop{\text{\normalfont\textsc{Tgt}}}}
\DeclareMathOperator{\ep}{\mathop{\text{\normalfont\textsc{Endpoints}}}}
\DeclareMathOperator{\srcidx}{\mathop{\text{\normalfont\textsc{SrcIdx}}}}
\DeclareMathOperator{\tgtidx}{\mathop{\text{\normalfont\textsc{TgtIdx}}}}
\newcommand{\card}[2][]%
%{\ifx&#1&\##2\else\left(\##2\right)^{#1}\fi}
{\ifx&#1&\##2\else{\##2}^#1\fi}
%{|#2|^{#1}}

\newcommand{\bigo}[1]{\mathbf{O}\mathopen{}\left(\rule{0pt}{.9em}#1\right)\mathclose{}}
\newcommand{\bigomega}[1]{\mathbf{\Omega}\mathopen{}\left(\rule{0pt}{.9em}#1\right)\mathclose{}}
\newcommand{\bigtheta}[1]{\mathbf{\Theta}\mathopen{}\left(\rule{0pt}{.9em}#1\right)\mathclose{}}
\DeclareMathOperator{\size}{\mathop{\text{\normalfont\textsc{Size}}}}
\DeclareMathOperator{\walks}{\mathop{\text{\normalfont\textsc{Walks}}}}
\DeclareMathOperator{\matches}{\mathop{\text{\normalfont\textsc{Matches}}}}

\DeclareMathOperator{\lbl}{\mathop{\text{\normalfont\textsc{Lbl}}}}
\DeclareMathOperator{\dom}{\mathop{\text{\normalfont\textsc{Dom}}}}
\DeclareMathOperator{\len}{\mathop{\text{\normalfont\textsc{Len}}}}

\newcommand{\Add}[2]{add~~#1~~to~~#2}
\newcommand{\AddAll}[2]{add all elements in~~#1~~to~~#2}

\newcommand{\orcidicon}[1][1.5ex]{\adjustbox{max height=#1, raise=\dimexpr ( #1 * 195 / 700 * -1)  \relax}{\includesvg{images/orcid.svg}}}
\newcommand{\orcidexponent}[2][1ex]{\adjustbox{raise=#1}{\href{#2}{\orcidicon}}}
\newcommand{\orcidfull}[1]{\href{#1}{\orcidicon[1.1em]~\texttt{#1}}}

\newcommand{\sem}[1]{\llbracket #1\rrbracket}

\newcommand{\aut}[1]{\langle#1\rangle}


\newcommand{\varname}[1]{\mathit{#1}}
\newcommand{\smashedcommentpar}[2][.5\linewidth]{\Comment{\smash{\parbox[t]{#1}{#2}}}}
\newcommand{\commentpar}[2][.5\linewidth]{\Comment{\parbox[t]{#1}{#2}}}

\makeatletter
\newcommand{\set}[2][]{\{#1{\kern1\nulldelimiterspace}#2{#1\kern1\nulldelimiterspace\}}}
\newcommand{\setst}{\@ifstar{\autosetst}{\paramsetst}}
\newcommand{\autosetst}[2]{\left\{\,#1\,\middle|\,#2\,\right\}}
\newcommand{\paramsetst}[3][]{#1\{\,#2\mathbin{#1|}#3{\,#1\}}}

\newcommand{\bag}{\@ifstar{\autobag}{\parambag}}
\newcommand{\autobag}[1]{\llbrace*#1\rrbrace*}
\newcommand{\parambag}[2][]{\llbrace[#1]#2\rrbrace[#1]}
\newcommand{\bagst}{\@ifstar{\autobagst}{\parambagst}}
\newcommand{\autobagst}[2]{\llbrace*\,#1\,\middle|\,#2\,\rrbrace*}
\newcommand{\parambagst}[3][]{\llbrace[#1]\,#2\mathbin{#1|}#3\,\rrbrace[#1]}

\newcommand{\llbrace}{\@ifstar{\leftllbrace}{\paramllbrace}}
\newcommand{\paramllbrace}[1][]{{#1\{\hspace*{-.25em}#1\{}}
\newcommand{\leftllbrace}{\left\lbrace\kern-3\nulldelimiterspace\middle\lbrace}
\newcommand{\rrbrace}{\@ifstar{\rightrrbrace}{\paramrrbrace}}
\newcommand{\paramrrbrace}[1][]{{#1\}}\hspace*{-.25em}{#1\}}}
\newcommand{\rightrrbrace}{\middle\rbrace\kern-3\nulldelimiterspace\right\rbrace}
\makeatother


\newcommand{\citeauthoryear}[1]{\protect\citeauthor{#1}, \protect{\citeyear{#1}}}
\newcommand{\urlfootcite}[1]{\nolinebreak\footnote{\protect\citetitle{#1}. \protect\citeurl{#1}}}

\usepackage[framemethod=TikZ]{mdframed}
%\newsavebox{\mybox}%\fbox{\usebox{\mybox}}
\newlength{\problemmargin}
\setlength{\problemmargin}{0pt} 
\newlength{\problempadding}
\setlength{\problempadding}{1ex}
\newlength{\problemsep}
\setlength{\problemsep}{.25ex}
\newlength{\problemtitlepadding}
\setlength{\problemtitlepadding}{1ex}
\newcommand{\problembullet}{\textbullet~~}
\newcommand{\problemfont}[1]{\textsc{#1}}
\makeatletter
\newenvironment{problem}[1]{
    
    \addvspace{.5\baselineskip\@plus.2\baselineskip\@minus.2\baselineskip}% Cc-Cv from acmart.cls
    
    \begin{mdframed}[%
        frametitle={\hspace*{\dimexpr\problemtitlepadding-\problempadding\relax}#1},
        frametitlefont=\large\sc,
        innerleftmargin=\problempadding,
        innerrightmargin=\problempadding,
        innerbottommargin=\problempadding,
        innertopmargin=\problempadding,
        frametitleaboveskip=\problemtitlepadding,
        frametitlebelowskip=\problemtitlepadding,
        leftmargin=\problemmargin,
        rightmargin=\problemmargin,
%    frametitlealignment=\centering,
        frametitlerule=true,
        frametitlebackgroundcolor=black!10,
        nobreak,
        roundcorner=0pt,
        linewidth=0.5pt,
        frametitlerulewidth=0.5pt,
        ]%
    \description[topsep=0pt,itemsep=\problemsep,labelindent=0cm,leftmargin=\widthof{\problembullet},font=~\textbullet~\normalfont]%
}{%
    \enddescription\end{mdframed}
    
    \addvspace{.5\baselineskip\@plus.2\baselineskip\@minus.2\baselineskip}% Cc-Cv from acmart.cls
}
\makeatother


\newcommand{\functionfont}[1]{\textsc{#1}}
\newcommand{\minarrow}{{\normalfont\textsf{MinArrow}}}
\newcommand{\comp}{{\normalfont\textsf{Comp}}}

